The Vector Meson Mass in Chiral Effective Field Theory

A brief overview of Quantum Chromodynamics (QCD) as a non-Abelian gauge field theory, including symmetries and formalism of interest, will precede a focused discussion on the use of an Effective Field Theory (EFT) as a low energy perturbative expansion technique. Regularization schemes involved in Chiral Perturbation Theory (\c{hi}PT) will be reviewed and compared with EFT. Lattices will be discussed as a useful procedure for studying large mass particles. An Effective Field Theory will be formulated, and the self energy of the \r{ho} meson for a Finite-Range Regulated (FRR) theory will be calculated. This will be performed in both full QCD and the simpler quenched approximation (QQCD). Finite-volume artefacts, due to the finite box size on the lattice, will be quantified. Currently known lattice results will be used to calculate the \r{ho} meson mass, and the possibility of unquenching will be explored. The aim of the research was to determine whether a stable unquenching procedure for the \r{ho} meson could be discovered. The results from the original research indicate that there is no such procedure because the \r{ho} mesons are unstable. Unless additional data involving lighter quark masses is available, an element of modelling is needed for successful unquenching.

==> code.tex <==
\chapter{Original Code}
\label{App:Programs}

\section{Driver Program}

\subsection{RhoMass.f90}

{\scriptsize
\verbatiminput{../../routines/program/RhoMass.f90}
}

\subsection{myKinds.f90}

{\scriptsize
\verbatiminput{../../routines/program/myKinds.f90}
}


\section{Simulation}
\label{app:simulation}
\subsection{sim.f90}

{\scriptsize
\verbatiminput{../../routines/program/sim.f90}
}


\section{QQCD Data Analysis}
\label{app:quenched}
\subsection{quenched.f90}

{\scriptsize
\verbatiminput{../../routines/program/quenched.f90}
}

\section{Full QCD Data Analysis}
\label{app:full}
\subsection{full.f90}

{\scriptsize
\verbatiminput{../routines/program/full.f90}
}

\section{Lattice QCD Routines}
\label{app:lattice}
\subsection{Latt.f90}

{\scriptsize
\verbatiminput{../routines/program/Latt.f90}
}


\section{Integration Routines}
\label{app:integration}
\subsection{myIntegrate.f90}

{\scriptsize
\verbatiminput{../routines/program/myIntegrate.f90}
}

\subsection{Integrands.f90}

{\scriptsize
\verbatiminput{../routines/program/Integrands.f90}
}


\section{Singular Value Decomposition}
\label{app:svd}
\subsection{svdreal.f90}

{\scriptsize
\verbatiminput{../routines/program/svdreal.f90}
}

\subsection{fitCurve.f90}

{\scriptsize
\verbatiminput{../routines/program/fitCurve.f90}
}

\subsection{datagen.f90}

{\scriptsize
\verbatiminput{../routines/program/datagen.f90}
}

